Graph Inductive Biases in Transformers without Message Passing

Transformers for graph data are increasingly widely studied and successful in numerous learning tasks. Graph inductive biases are crucial for Graph Transformers, and previous works incorporate them using message-passing modules and/or positional encodings. However, Graph Transformers that use message-passing inherit known issues of message-passing, and differ significantly from Transformers used in other domains, thus making transfer of research advances more difficult. On the other hand, Graph Transformers without message-passing often perform poorly on smaller datasets, where inductive biases are more crucial. To bridge this gap, we propose the Graph Inductive bias Transformer (GRIT) -- a new Graph Transformer that incorporates graph inductive biases without using message passing. GRIT is based on several architectural changes that are each theoretically and empirically justified, including: learned relative positional encodings initialized with random walk probabilities, a flexible attention mechanism that updates node and node-pair representations, and injection of degree information in each layer. We prove that GRIT is expressive -- it can express shortest path distances and various graph propagation matrices. GRIT achieves state-of-the-art empirical performance across a variety of graph datasets, thus showing the power that Graph Transformers without message-passing can deliver.

==> Sections/background.tex <==

\newcommand{\liheng}[1]{\textcolor{maroon}{#1}}


\section{Background}


Following the success of Transformers~\citep{vaswani2017AttentionAllYou} in different modalities like natural language processing~\citep{vaswani2017AttentionAllYou} and computer vision~\citep{dosovitskiy2020ImageWorth16x16}, 
much recent work has focused on developing Transformers for graph data~\cite{dwivedi2021GeneralizationTransformerNetworks, kreuzer2021RethinkingGraphTransformers, ying2021TransformersReallyPerform, wang2021GraphStructureAware, hussain2022GlobalSelfAttentionReplacement, rampasek2022RecipeGeneralPowerful}. 


Various graph Transformers have achieved state-of-the-art empirical results, including in major challenges such as the Open Graph Benchmark Large Scale Challenge (cite ogb-lsc). The particular structure and symmetries of graph data call for certain modifications to the Transformer architectures used in other domains --- for instance, there is no ordering or coordinate system for nodes in a graph as there are for text in a sequence or pixels in a grid.

However, many current graph transformers are still retaining the (local) message-passing mechanism --- the key component of most graph neural networks (GNNs) --- in their architecture~\cite{dwivedi2021GeneralizationTransformerNetworks, kreuzer2021RethinkingGraphTransformers}.
While message-passing has many benefits, it also has known limitations, so these graph Transformers inherit such limitations. 
For instance, message-passing GNNs (MPNNs)~\cite{kipf2017SemiSupervisedClassificationGraph, hamilton2017InductiveRepresentationLearning, xu2019HowPowerfulAre, velickovic2018GraphAttentionNetworks, bresson2018ResidualGatedGraph, hu2020StrategiesPretrainingGraph, corso2020PrincipalNeighbourhoodAggregation} are known to be limited in expressive power, sometimes prone to oversmoothing, and limited in capturing long-range interactions. Moreover, the message-passing in many graph Transformers makes these Transformers quite different from those used in other data domains; this hinders graph Transformers from fully leveraging the advances made in the massive body of Transformer research in other fields.

\textcolor{red}{
A recent study~\cite{rampasek2022RecipeGeneralPowerful} has revealed that integrating graph transformers with MPNNs can effectively boost the empirical performance, hinting that the current graph transformers cannot completely substitute MPNNs on graph learning.
}



In this work, we introduce a new graph Transformer without message-passing. Key to our method is the use of relative positional encodings based on random walk probabilities. Moreover, \ldots, so we incorporate degree scalars that inject degree information into our Transformer (TODO: add justification). We choose a particular form of attention that allows us to successfull incorporate our relative positional encodings.

To justify our architecture, we prove that it can express shortest path distances, thus generalizing other graph Transformers like Graphormer and (cite others). Further, we demonstrate state-of-the-art performance in numerous graph datasets. Ablation studies empirically justify our architectural choices.


\section{Related Work}

graph transformers with no message-passing: graphormer, jinwoo kim's works, biconnectivity paper. note that shortest paths can be expressed in our framework

Several graph Transformers without message-passing have been proposed. The most notable one is Graphormer~\citep{ying2021TransformersReallyPerform}, which won the graph regression task of the 2021 OGB Large Scale Challenge; Graphormer uses all-pairs shortest path distances as a relative positional encoding in a standard Transformer. However, our model outperforms these graph Transformers, bringing non-message-passing Transformer performance back in line with the hybrid graph Transformers that have recently been outperfoming them.

Many other hybrid graph Transformers that include message-passing have been developed.

other graph transformers: graphgps, SAN, mialon, dwivedi, sat, egt, etc

Positional encodings on graphs have to be quite different from those of other domains, since nodes of graphs do not come with explicit coordinates. Thus, there have been many proposed positional encodings on graphs, that are permutation equivariant or nearly permutation equivariant. Most similarly to our relative random walk positional encodings, \citet{dwivedi2021GraphNeuralNetworks} and \citet{li2020DistanceEncodingDesign} propose random walk structural encodings. The former uses only node structural encodings for GNNs and graph Transformers, and the latter uses relative encodings as edge weights within GNNs; in our method, we use the full random walk probability matrices as relative positional encodings within Transformers. There are also other positional encodings based on heat kernels on graphs~\citep{mialon2021GraphiTEncodingGraph, feldman2022weisfeiler}. Many methods use Laplacian eigenvectors as node positional encodings~\citep{dwivedi2020BenchmarkingGraphNeural, dwivedi2021GeneralizationTransformerNetworks, kreuzer2021RethinkingGraphTransformers, dwivedi2022LongRangeGraph, kim2022PureTransformersAre, lim2022SignBasisInvariant}, though this generally necessitates dealing with the symmetries of eigenvectors~\citep{lim2022SignBasisInvariant}.



\textcolor{red}{to add:
Positional-structural encoding schemes have been demonstrated valid to enhance the expressive power of GNNs and GTs, theoretically~\cite{loukas2020WhatGraphNeural} and empirically~\cite{dwivedi2022BenchmarkingGraphNeural, dwivedi2021GeneralizationTransformerNetworks, kreuzer2021RethinkingGraphTransformers, dwivedi2021GraphNeuralNetworks, rampasek2022RecipeGeneralPowerful}}



